Rethinking and Recomputing the Value of Machine Learning Models

In this paper, we argue that the prevailing approach to training and evaluating machine learning models often fails to consider their real-world application within organizational or societal contexts, where they are intended to create beneficial value for people. We propose a shift in perspective, redefining model assessment and selection to emphasize integration into workflows that combine machine predictions with human expertise, particularly in scenarios requiring human intervention for low-confidence predictions. Traditional metrics like accuracy and f-score fail to capture the beneficial value of models in such hybrid settings. To address this, we introduce a simple yet theoretically sound "value" metric that incorporates task-specific costs for correct predictions, errors, and rejections, offering a practical framework for real-world evaluation. Through extensive experiments, we show that existing metrics fail to capture real-world needs, often leading to suboptimal choices in terms of value when used to rank classifiers. Furthermore, we emphasize the critical role of calibration in determining model value, showing that simple, well-calibrated models can often outperform more complex models that are challenging to calibrate.

==> sections/confidence.tex <==
\section{The centrality of joint confidence-accuracy distributions}
% We now get back to our initial assumption that rejection is implemented by filtering items where the prediction confidence is lower than a threshold. So, we have a model $m$ and apply our simple selector $s$ to obtain $g$, given a threshold $\tau$.
% This means that we can now talk in terms of $V(m,t,D)$ since we can compute $g$ given $(m,t)$.

% Given a value of $k$ and a tuning dataset, we can solve an optimization problem to derive the threshold. There are many ways in which this can be done or approximated, and in most cases the problem is trivial practice.
% This means that given a dataset, $\tau$ is a function of $k$.
% Equation \ref{eq:simplevaluek} may be frustrating: We are used to work with accuracy and now we have to live with these parameters that, in addition, depend on the threshold. Perhaps accuracy, precision, recall, F1, and so on are good approximations that lead us to learning good models, and we can do even better if we try to keep ECE low.
To see why thinking in terms of value does matter, both in theory and in practice,we begin by asking two questions, or, two sides of the same question:
given two models, which one is "better"? And, given iterations of a training algorithm, when can we say that the algorithm is "learning"?
The first question is trivial if we have the use case, that is, we know the value function and have a tune and test dataset: we can pick the best model empirically, under the usual i.i.d. assumptions commonly made for the representativeness of tune or test datasets.
However, we often do not have the value function because we are training or assessing models to cover a variety of use cases and cost functions. This is a common need - think of a sentiment classifier or a language detector: they are often developed to work for a variety of use cases. 

One way to assess models is to plot $V(m,\calD,k)$ over $k$ (remember that given $m$, $\calD$ and $k$ we can obtain $\tau$). By doing this we could find that one model always has higher value, and as such is "Pareto-better".
Alternatively, we could define some notion of "area under the value curve" and take that - or a subset in some meaningful range of $k$.
This is useful, but does not give us much insights on what it means to learn, what is a "good" model, and what is the (active) learning strategy we should use.

\subsection{Weaknesses of commonly accepted metrics and methods}
Metrics such as accuracy and precision are often used to assess and compare models. In case where filtering by confidence is important, ECE is often used ~\cite{Guo2017CalibrationOfMNNs}. 
A trivial example, shown in Figure \ref{fig:pdf} explains why this does not work. 
Model $m1$ always predicts with confidence (for the highest confidence class) of 0.6, and also has an accuracy of 0.6.
Model $m2$ has a lower overall accuracy 0.5 but for half of the items (say, images with a white background) it emits a top confidence of 0.9 - and also has 0.9 accuracy for those, while for the other half  it has confidence and accuracy of 0.1. Model $m3$ is similar for white backgrounds, but on the other half of the images it predicts at 0.3 accuracy (and 0.3 confidence).

All three models are perfectly calibrated. $m3$ has the same accuracy of $m1$ and $m2$ has \textit{worse} accuracy, but both deliver better value for a wide range of $k$, and specifically for $k>1.5$ (which puts the threshold over 0.6 for our perfectly calibrated models, recall $\tau>k/(k+1)$ in this case). \andrea{I would add a plot with the values of the three models as functions of $k$, side-by-side with this one (they can stay on a single column)}

\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{figs/pdf.png}
\caption{Probability density function (impulses in this case) for three models over a dataset}.
\label{fig:pdf}
\end{figure}

% why accuracy and calibration - as defined in the literature -  

% We first discuss why commonly used metrics. The discussion above has already shown that accuracy is the value of a model at $\tau=0$.
% In other words if we optimize for accuracy we optimize for a special case, and as shown in fig XX (and later in the experiments) models with same accuracy can have very different values.
% The same is true for ECE, also from figure XX. 




\subsection{Accuracy-based calibration error}
The problem with ECE, and with all commonly used measures of calibration is i) that they predicate on accuracy $A$ given  confidence  $C$ (essentially, assess how far $P(A|C)$ is from $C$, in expectation) and ii) they neglect value.
A doctor that assesses the probability of you having a disease based on the national statistics on patients, without competence or examination (say, 5\% have the flu in winter so your probability of having the flu is stated at .05) has zero ECE. Yet, it is useless. 
Even in cases where we do not have ECE=0 and we improve it, it may not make a difference - in fact, we can have models $m_1$ and $m_2$ with same accuracy and where the model with worse ECE has better value. In our example, just tweak a little $m3$ to make it slightly underconfident or overconfident for the impulse at 0.3: you have higher ECE but still higher value for most values of $k$.
% The challenge with the measures of calibration is that they tend to measure average accuracy given a confidence. In other words, they predicate about $P(A|C) $. 

We argue that predicating on $P(A|C)$  is not very helpful in itself, and what we need to look into, if we could, is $P(A,C)$ and $P(C|A)$.
Indeed, once we fix a threshold $\tau$, we want to:
% maximize $P(Y = \hat{Y} | C > t)$ and minimize $P(Y = \hat{Y} | C < t)$. 
% So we want to:

Maximize $P(Y = \hat{Y} | C > \tau) = \frac{P(Y = \hat{Y} , C > \tau)}{P (C > \tau)} = \frac{P(C > \tau | Y = \hat{Y} ) P(Y = \hat{Y})}{P (C > \tau)}$


Minimize $P(Y = \hat{Y} | C < \tau) = \frac{P(Y = \hat{Y} , C < \tau)}{P (C < \tau)} = \frac{P(C < \tau | Y = \hat{Y} ) P(Y = \hat{Y})}{P (C < \tau)}$

% $P(y = \hat{Y} | c < \tau) = P(y = \hat{Y} , c < \tau) / P (c < \tau)$
This is true regardless of which $\tau$ we choose, and different value functions will lead to different optimal $\tau$. 
In the dream world we look for models that assign a confidence of 1 when they are correct, and a confidence of $1/|\calY|$ (which is the minimal confidence when $|\calY|$ is the number of classes) when they are wrong.
In practice this is hard to achieve but we want models that go in this direction, that is, \textbf{we expect that if we have two samples $\calD_1$ and $\calD_2$, if the model accuracy is greater on $\calD_1$, then the average confidence is also greater} (again, in expectation).
% To see this, imagine that you have a model $m$ that emits predictions $\hat{Y}$ and confidences $\hat{C}$ (for the top level predictions $\hat{Y}$) over a dataset $\calD$.
% \calDenote as $\chi_\calD$ the set of possible assignments of confidences obtained without changing $\hat{Y}$ (and so without changing accuracy) - or equivalently, consider all the set of models that are prediction-equivalent to $m$. What we ideally want to look for is for the set of confidence assignments (models) such that:




% \textbf{Representativeness of confidence values. xxx need better term}

The above shows that the quality of a model depends on its joint distribution of confidence and accuracy. 
The challenge we face is that defining this distribution is tricky. We want to think in terms of  $P(C|A)$ and $P(C)$, but conditioning on accuracy is hard, since there is no accuracy associated to an item: A prediction is either correct or wrong (at least that is how we model reality in this paper). 
% And, if we take large iid samples from $\calD$ we are back to square 1: we are ok to have meaningless, non discriminative confidence measures as for large samples a model with confidence equal to average accuracy will show good "calibration".
However, we can sample among possible item sets $\calD_{n,a}$ of size $n$ for which the accuracy at threshold zero  is $a$ ($\alpha_0=a$). 
In other words, instead of bucketing by confidence as we do when we compute ECE, we "bucket by accuracy". 


Once we have the notion of samples of size $n$, then we can obtain a set of $\calD_1,..\calD_N$ samples, each of size $n$, compute for each the accuracy and average confidence, and use that to compute an accuracy-binned expected calibration error (ABECE) where we bin by accuracy: given a sample size $n$, we have $n+1$ possible accuracy values for each sample, and so n+1 bins.
We can then take a set of samples, compute the accuracy for each, and place the points in each sample $s$ in the bin corresponding to the accuracy. 

With this, we can compute E[C|A)], meaning, given an accuracy bucket we can derive the expected confidence, and we can also compute $E[R_n = C - A | A]$.
We can compute variants of accuracy-based calibration error by summing the absolute value of the error $R_n$ across buckets, or by weighing the sum by mass in that bucket (similarly to what  ECE does~\cite{Naeini2015}\footnote{Because we obtain buckets by sampling, while we can do this we need to be mindful that larger size buckets will tend to move mass towards the overall mean accuracy, so while possible it may be a less informative metrics.}).

If buckets are thin, then it is easy to see that having average confidence match accuracy is "valuable" in terms of value function. 
If we consider the points in a (narrow) accuracy bucket $a$, and given a threshold $\tau$ used for selection, any time $a$ and $\mu_c$ for that bucket are on the opposite side of t (eg, $a>t$ and $\mu_c<t$) then we miss out, that is, the value would be higher if the confidence was brought up (or down) to be closer to $a$.

\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{figs/abece.png}
\caption{Binning by accuracy shows how poor m1 is}.
\label{fig:abece}
\vspace{-0.15in}
\end{figure}

  

% To reason about the kind of behavior we want from a model, consider a random variable $R_n = \mu_c - \alpha_0$, defined as the difference between the average confidence of a model $m$ and the accuracy over a sample of size $n$.
% % ECE=0 over a dataset $\calD$ implies that $E[R]=0$ only for the sample has $n=|\calD|$ or for samples that coincide with the ECE bucketing. 


% In this case, we wish to have $\mu_c=a$ and $E[R_{n,a}]=0$. 

\subsection{Learning and calibration}
Accuracy-based measures of calibration errors are interesting because related to value as shown above. However, there are other representations stemming from the same concepts that are useful to understand what "learning" means or how to drive an (active) learning process. 
For example, while ABECE predicates on P(C|A), we can plot the joint probability density function $f_n(a,\mu_c)$ using the same method: we bin by both accuracy and confidence, and then each sample of size $n$ ends in one square bucket only (Fig.~\ref{fig:learning}).
Similarly, we could bucket by features of the domain space and compute $R_{n}$ for each bucket. For example, we can bucket by features (e.g., by language of a text, or background color of an image, or any separation of the domain) and desire that $R_{n}$ be small for each bucket $b$.
% Notice that while the confidence axis is continuous and $\mu_c$ can take any value in $[0,1]$, on the accuracy axis the possible values are $n+1$.
% Similarly, we can study the pdf of random variable $R$, which again can be computed having (confidence, accuracy) as domain, or based on any other bucketization of interest.
% One special case is where we bucketize based on confidence only, and in that case are back to ECE-style metrics.




% When we do this, 
% that is defined for a model $m$ over a sample $n$ of items, and has as 
% So the key here is that we want to be able to define notions of "sample of size $n$" that are not iid / random sample from $\calD$ but where still $E[R]=0$.
% Specifically,  In this case, 



Given m, and value function, we can compute $E[V(m,D)]$. 
If we reason in terms of joint distributions, given a threshold $\tau$ on confidence we can compute both $\rho_t$ - which is the area below t considering only the marginal distribution of confidence - and $\alpha_t$, which is the area of $f$ above $\tau$ considering only the marginal distribution of accuracy.

Now, if we consider learning as improving the value of a function, either for a given $k$ or for any $k$, then we can see that learning can take at least three shapes: one is obvious and has to do with improving accuracy (shifting mass \textit{vertically}, up in the density chart - blue arrows in Fig.~\ref{fig:learning}).
Notice that this worsen the value of $R$ for each cell, but improving accuracy keeping everything else unchanged always leads to same or higher value. Notice also that the left blue arrow does not bring value: it improves accuracy but keeps the points below threshold\footnote{This is not always true since we set the threshold based on a tuning set, so if the increase in accuracy is large and close to the threshold, $\tau$ would actually move left}. 
If we do not touch accuracy (we do not change the inferences made by the model in terms of $\hat{Y}$), we can still learn by shifting mass \textit{horizontally} towards the diagonal (red arrows in Fig.~\ref{fig:learning}) - which essentially means better calibration.
The third one has to do with "breaking bricks": even if the overall accuracy does not improve and we do not move horizontally towards the diagonal, we can take a set of items that in a previous learning iteration were similar in terms of our confidence and accuracy and learn to discriminate among some for which we can have higher confidence and accuracy, and others for which we have lower confidence and accuracy (orange arrows in Fig.~\ref{fig:learning}). Notice that here too some leanings may provide value to a use case (cross a threshold), while others do not.
In general every learning cycle is likely to be a mix where multiple effects combine together.


\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{figs/learning.png}
\caption{Example joint density function (darker values denote higher values). The arrows represent three possible types of learning, and the black line is an hypothetical threshold for a selective classifier}.
\label{fig:learning}
\vspace{-0.15in}
\end{figure}



From the above we can derive two observation: first, \textbf{we can arrive at a notion of calibration gain, which is an increase of value obtained} without changing the top level prediction (and therefore \textbf{without changing accuracy}).
In other words, if we have two models $m_1$ and $m_2$ that make the same inferences (same $\hat{y}$ for every $x \in \calD$), then 
$G = V(m_2,\calD,k) - V(m_1,\calD,k)$ represent the gain due to calibration. 
Second, we observe that since calibration increases value, then calibration is part of learning just as improving accuracy is,
much like when by studying a subject further we become more aware of what we know and more aware of what we do not know, as Socrates used to teach us ~\cite{plato}. And both the second and third form of learning can achieve that.

% If we start from a model $m$ and we obtain a model $q$ that has the same accuracy (same $\alpha_0 = P(y = \hat{y}$), but can "move" confidences of some correct examples above the threshold, it will always increase value (for any value function), and the same is true if $q$ reduces the confidence of an incorrect one. (\textbf{xxx to show}).
% What this is telling us is that "learning", aside from improving accuracy, can be obtained by either increasing the confidence of examples for which we classify correctly, or decreasing the confidence of what we predict incorrectly.
% This increase value, so it is a learning, much like when by studying a subject further we become more aware of what we know and more aware of what we do not know, as Socrates used to teach us.



% In general - unless we know $\tau$ in advance, this means that we want to "spread" our confidence measures as much as possible and ideally push them away from $\tau$.


% In other words, what we want from our confidence function is that if on an arbitrarily selected and arbitrarily small dataset $\calD$ the average accuracy is right, the confidence should reflect that. 
% The only "limit" to the size of $D$ is that a prediction is either right or wrong, so the only way to assert the extent to which confidence measures are representative of what a model actually knows is to compute accuracy over $n$ samples.





% To describe how we think about measures of how "meaningful" are confidence measures and the properties of a "good" model, we follow an approach  based on defining random variables and their properties.

% In principle, a good property would seem to be the following:  consider a dataset $D$, and a sample of size $n$ from $D$.
% The difference between the accuracy $ R=\mu_c(D)-\alpha_0(D)$ (where $\mu_c(D)$ is the mean confidence), is a random variable.
% In general, it is desirable to have $E[R] = 0$.
% However, this is not per se essential. 
% Since we can set the threshold based on a tuning set, we can live with average over or under estimation - the limitation is that the tuned threshold is not representative of a "probability".



% In this framework, the ECE and variations measure the empirical $\mu_R$ over a set of $b$ datasets, where $b$ is the number of bins and the datasets $D_1,\dots,D_b$ are selected based on the confidence range of their items.
% A model with ECE=0 also has $\mu_R=0$ and $\mu_S=0$, \textit{but only over the bins that define the ECE}, which condition over confidence value. In other words, ECE measures, and even notions of perfect calibration, condition error definition on the prediction confidence. 

% \textit{But the problem is that we do not "just" care of the P(accuracy | confidence): the essence of learning and of model quality is in the joint probability P(accuracy, confidence) over the data.}
% If we have a subset of a dataset for which the accuracy is high, we want the confidence to be high so they are above threshold and we can get value. And the opposite holds if accuracy is low. This is why $P(C|A)$ is important. 





% This is the key: if we sample items to build sets $D_{n,a}$ of size $n$ for which the model has accuracy $a$, then we expect $\mu_c=a$.



% In other words, for any $a$, we expect E[R_{]


% on  Instead, given a dataset $D$ there are many cases where $\mu_S\neq 0$ while ECE=0.

% We want confidence value to be representative of what the model knows, that is, be a good description of what it knows: it should not over-represent it or under represent it, for each item.
% Neither ECE nor the notion of perfect calibration capture this property. What existing measures do is to predicate about accuracy given the confidence. \textbf{xxx say why}.
% So the problem with both ECE and perfect calibration is that they predicate in various ways over $P(A|C)$ and the random variable $A_C = A | C$, the conditional probability of the accuracy of a sample given the confidence (and specifically the expectation is that $E[A_C]=C$).
% The limitation is that we do not care that much about $P(A|C)$.


% m = f(A,C) where f is a joint probability density function over a domain $D$. 




% Given this, what does it mean to learn?
% of course we can learn by pushing accuracy towards 1. 
% Increasing the accuracy for any point of $f$ will always result in a more valuable model.
% However, we can "learn" without touching the accuracy distribution at all, and even without touching P(A|C).
% Ideally, given an overall accuracy $\alpha_0(D)$, we want to see mass on the diagonal.
% For example, a learning iteration may be such that we do not increase our accuracy overall,  we do not improve our ECE overall (we can even assume we are always perfectly calibrated according to the definition of xxx), but we shift the joint density function to have higher values in the bottom left and top right corners of the (confidence, accuracy) space.

% Another way to see this is that learning has to do with pushing confidences apart: we can have a data subset SD for which m gives the same confidence $c$ and accuracy $\alpha(SD)$, and learning means separating this set SD into subsets $SDA$ and $SDB$ for which  $\alpha(SDA) > \alpha(SDB)$ (even if $\alpha(SD) >\alpha(SDB)$, so we actually do worse on some points, and $\mu_c(SDA) > \mu_c(SDB)$. 



% What we really care about is that if, given two sets $D_1$ and $D_2$, and renaming as DH the dataset of the two with higher accuracy and with DL the one with lower accuracy (so that  $\alpha_0(DH) \geq \alpha_0(DL)$), 
% then we \textit{expect} $\mu_c(DH) \geq \mu_c(DL)$. 
% In fact, the larger the difference in accuracy the larger we want the difference in confidence to be. 
% So in general if we define random variables $A=\alpha_0(DH) - \alpha_0(DL)$ and $M_c=\mu_c(DH)- \mu_c(DL)$, and we define $S=A-M_c$, then we want  $E[S] = 0$ and the standard deviation to be "small" (remember that we are taking as $D_1$ the set with the higher accuracy, which means that ).
% Notice that $S$ may equivalently be written as $S(DH,DL)= R(DH) - R(DL)$. 

% For simplicity we can assume that the datasets are of the same size $n$, and we can then talk about random variable $S_n$, and mean and standard deviation $\mu_{S_n}$ and $\sigma_{S_n}$.

% \bigskip



% 1. calibration, in the sense that given a randomly selected dataset $D$, we want $\alpha(D) ~ \mu_c(I_1)

% 2. discrimination: if we take two random sets of items $I_a$ and $I_b$, if $\alpha_0(I_1) > \alpha_0(I_2)$ then we \textit{expect} that $\mu_c(I_1) > \mu_c(I_2)$, where $\mu_c$ is the average confidence on a dataset.

% The above raises the question about the difference between calibration and learning. In the end it is a matter of definition. We could define calibration as a process that only moves density horizontally, towards the diagonal, or any process that changes confidence measures without changing accuracy.
% In general, given a model $m$ that returns certain predictions over a dataset $D$, we can define  calibration error at $K$ as the difference in value between V(m,K) and the model $q$ such that $m$ and $q$ return the same $\hat{y}$ but that has the maximum value.   
% \textbf{xxx this we need to think through a bit. }

% Given the above, we can think at the classes of models that return the same predictions (and so they have also the same accuracy).


% We refer to confidence calibration as the process of changing confidence values to obtain a model that has higher value.  

% and define the calibration error in terms of... distance from the diagonal? difference in value 

% define as expected calibration error the distance from the diagonal in value that a calibrated model 


% Notice that you can have a calibrated model that is arbitrarily bad. An untrained model that only knows the class distribution may "simply" return a confidence vector that mirrors the distribution, and this is a perfect representation of the model's knowledge - the model cannot do better.









% Let us denote with $\alpha_t$ the accuracy for predictions above a threshold $\tau$.
% Accuracy as typically computed (on all items) is then $\alpha_0$ since it is akin to setting a confidence to 0 (or less, which doesn't make sense but is mathematically possible).
% $V(m,0,D) =  \alpha_0 (k+1) -k$

% xxx plot shows when the difference matters.
% xxx plot v0 vs alpha for values of k (or vice. versa), and v0 vs vt

% Now, assume we are given a threshold $\tau$, and let us consider the question of when a model $m_1$ is better (higher value) than a model $m_2$, even if they have the same accuracy ($\alpha_{0,a}  = \alpha_{0,b}$). 
% Our guide here is equation \ref{eq:expectedvalue}


% \begin{enumerate}
% \item $\rho$ is identical for the two models ($\rho^t_a=\rho^t_b$), but $m_a$ is more accurate for prediction that have confidence above the threshold (and therefore less accurate below the threshold since $\alpha^0$ is the same - but accuracy below threshold does not affect value). 
% So, $\alpha_{t,a}  > \alpha_{t,b}$.
% Notice that if $\rho_{t,1}=\rho_{t,b}$, then $\alpha_{t,a}  > \alpha_{t,2} \implies E[V_{t,a}] > E[V_{t,b}]$
% \item Alternatively, accuracy above threshold can be identical but $\rho$ may differ.
% This case is interesting since, under this assumption, $E[V_{t,a}] - E[V_{t,b}] =\rho_{t,a} (k-1 -\alpha_t(k+1)) - \rho_{t,b} (k-1 -\alpha_t(k+1)) $ 


% \end{enumerate}



% Next, we show that models with the same accuracy and calibration errors can lead to very different value function.


% \noindent \textbf{Active learning and certainty sampling.}
The joint distribution does not have to be built by bucketing based on accuracy. In fact a more useful way to do so is to bucket by areas in the feature space - for example, separate images based on the prevailing background color.
When we do so, we can identify areas of the domain where we do not perform as well as we should (in terms of $R$). We can do so regardless of a value function (if that is unknown), or mindful of it, if we know $V()$.
When we are mindful of the value function or of a threshold, then what matters to improve the value is to push correct classifications above the threshold and incorrect ones below. 
Since this is the goal, uncertainty sampling may not be the way to go. 
On the contrary, we may focus on squares closer to the confidence threshold, or on "bricks" that we can more effectively break because they are more "learnable" (how to find this out is a separate issue).
Indeed, when the cost of errors is high, uncertainty sampling may be the exact opposite of what we want to do.


% xxx add thoughts here



